Beyond the Black Box: A Survey on the Theory and Mechanism of Large Language Models

The rapid emergence of Large Language Models (LLMs) has precipitated a profound paradigm shift in Artificial Intelligence, delivering monumental engineering successes that increasingly impact modern society. However, a critical paradox persists within the current field: despite the empirical efficacy, our theoretical understanding of LLMs remains disproportionately nascent, forcing these systems to be treated largely as ``black boxes''. To address this theoretical fragmentation, this survey proposes a unified lifecycle-based taxonomy that organizes the research landscape into six distinct stages: Data Preparation, Model Preparation, Training, Alignment, Inference, and Evaluation. Within this framework, we provide a systematic review of the foundational theories and internal mechanisms driving LLM performance. Specifically, we analyze core theoretical issues such as the mathematical justification for data mixtures, the representational limits of various architectures, and the optimization dynamics of alignment algorithms. Moving beyond current best practices, we identify critical frontier challenges, including the theoretical limits of synthetic data self-improvement, the mathematical bounds of safety guarantees, and the mechanistic origins of emergent intelligence. By connecting empirical observations with rigorous scientific inquiry, this work provides a structured roadmap for transitioning LLM development from engineering heuristics toward a principled scientific discipline.

==> MainTex/taxonomy.tex <==
% --- 样式定义 ---
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-black,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
]
\tikzstyle{leaf}=[
    my-box, 
    minimum height=1.5em,
    fill=yellow!32, 
    text=black,
    align=left,
    font=\normalsize,
    inner xsep=5pt,
    inner ysep=4pt,
    align=left,
    text width=28em,
]
\tikzstyle{leaf2}=[
    my-box, 
    minimum height=1.5em,
    fill=purple!27, 
    text=black,
    align=left,
    font=\normalsize,
    inner xsep=5pt,
    inner ysep=4pt,
]
\tikzstyle{leaf3}=[
    my-box, 
    minimum height=1.5em,
    fill=hidden-blue!57, 
    text=black,
    align=left,
    font=\normalsize,
    inner xsep=5pt,
    inner ysep=4pt,
]

\newcommand{\eg}{\textit{e.g.}, }
\newcommand{\cit}[1]{[#1]}

\begin{forest}
    forked edges,
    for tree={
        grow=east,
        reversed=true,
        anchor=base west,
        parent anchor=east,
        child anchor=west,
        base=left,
        font=\large,
        rectangle,
        draw=hidden-black,
        rounded corners,
        align=left,
        minimum width=4em,
        edge+={darkgray, line width=1pt},
        s sep=3pt,
        inner xsep=2pt,
        inner ysep=4pt,
        line width=1.1pt,
        ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
    },
    % --- 层级宽度调整 ---
    where level=1{text width=9em,font=\normalsize,}{}, % Stage (Data, Model...)
    where level=2{text width=11em,font=\normalsize,}{}, % Topic (Mixture, PEFT...)
    where level=3{text width=48em,font=\normalsize,}{}, % Leaf (Citations)
    % ================= 内容部分 =================
    [LLM Theory \\ \& Mechanisms, ver
        % --- Stage 1: Data (使用 leaf 黄色) ---
        [\ \ Data Preparation\\ \ \ (\S 2), ver
            [\ \ \ Data Mixture
                [\eg Data Mixing Laws \cit{345}{,} BiMix \cit{77}{,}\\ DoReMi \cit{321}{,} DOGE \cit{64}{,} ScaleBIO \cit{227}{,}\\ RegMix \cit{188}{,} UtiliMax \cit{110}{,} Zakerinia et al. \cit{359}, leaf]
            ]
            [\ \ \ Deduplication \& \\ \ \ \ Filtering
                [\eg MinHash LSH \cit{133}{,} FED \cit{279}{,} D4 \cit{292}{,} SoftDedup \cit{107}{,} Lee et al. \cit{164}{,} Kandpal et al. \cit{147}{,} RefinedWeb \cit{232}, leaf]
            ]
            [\ \ \ Memorization
                [\eg Mosaic Memory \cit{273}{,} ACR \cit{264}{,} Memorization Sinks \cit{80}{,} Scaling Laws \cit{196}{,} Entropy Law \cit{127}{,} PEARL \cit{53}, leaf]
            ]
            [\ \ \ Synthetic Data
                [\eg Reverse-bottleneck \cit{71}{,} Curse of Recursion \cit{275}{,} Model Collapse \cit{55, 220}{,} Parrot Dilemma \cit{213}{,} Seddik et al. \cit{265}, leaf]
            ]
        ]
        % --- Stage 2: Model (使用 leaf2 紫色) ---
        [\ \ Model Preparation\\ \ \ (\S 3), ver
            [\ \ \ Representability
                [\eg Universal Approx. \cit{358}{,} Turing Completeness \cit{235, 47}{,} Bounded Dyck \cit{339}{,} Circuit Complexity \cit{209}{,} Lower Bounds \cit{32}, leaf2]
            ]
            [\ \ \ Theoretical Design
                [\eg Sparse Rate Reduction \cit{353}{,} Info Bottleneck \cit{378}{,} Energy Transformer \cit{117}{,} Hopfield Networks \cit{243}{,} Test-Time Training \cit{282}, leaf2]
            ]
            [\ \ \ Linear \& Recurrent
                [\eg RetNet \cit{283}{,} RWKV \cit{234}{,} Mamba \cit{88}{,} TTT \cit{302}{,} Looped Transformers \cit{332, 65}{,} Ouro \cit{385}{,} PLT \cit{315}, leaf2]
            ]
        ]
        % --- Stage 3: Training (使用 leaf3 蓝色) ---
        [\ \ Training Stage\\ \ \ (\S 4), ver
            [\ \ \ Scaling Laws
                [\eg Chinchilla \cit{116}{,} Data-Constrained \cit{154}{,} Emergence \cit{319}{,} U-Shaped Scaling \cit{319}{,} Intrinsic Dimension \cit{101}, leaf3]
            ]
            [\ \ \ Optimization
                [\eg $\mu$P \cit{331}{,} Step Law \cit{168}{,} Adam Convergence \cit{370}{,} Heavy-tailed Noise \cit{365}{,} Muon \cit{184}{,} Galore \cit{373}, leaf3]
            ]
            [\ \ \ PEFT Tuning
                [\eg LoRA \cit{121}{,} DoRA \cit{190}{,} LoRA+ \cit{103}{,} Adapter Asymmetry \cit{384}{,} Subspace Optimization \cit{373, 108}{,} Prompt Tuning \cit{236}, leaf3]
            ]
        ]
        % --- Stage 4: Alignment (使用 leaf 黄色) ---
        [\ \ Alignment Stage\\ \ \ (\S 5), ver
            [\ \ \ Safety Limits
                [\eg Alignment Impossibility \cit{314}{,} Shallow Safety \cit{238}{,} Likelihood Displacement \cit{244}{,} Elasticity \cit{138}{,} Recursive Curation \cit{63}, leaf]
            ]
            [\ \ \ Weak-to-Strong
                [\eg W2SG \cit{22}{,} Misfit Error \cit{29, 341}{,} Bias-Variance \cit{324}{,} Superalignment \cit{222}{,} Scalable Oversight \cit{20}, leaf]
            ]
            [\ \ \ RL Mechanisms
                [\eg RLVR \cit{357}{,} Echo Chamber \cit{374}{,} ProRL \cit{186}{,} Reward Hacking \cit{69, 75}{,} RTO \cit{376}{,} Markovian Thinking \cit{2}, leaf]
            ]
        ]
        % --- Stage 5: Evaluation (使用 leaf2 紫色) ---
        [\ \ Evaluation Stage\\ \ \ (\S 7), ver
            [\ \ \ Benchmarks
                [\eg Item Response Theory \cit{379}{,} Social Choice \cit{362}{,} Shortcut Learning \cit{59}{,} Benchmark Saturation \cit{379}{,} Difficulty Ceiling \cit{806}, leaf2]
            ]
            [\ \ \ Trustworthiness
                [\eg Hallucination Inevitability \cit{328}{,} Knowledge Overshadowing \cit{369}{,} Watermarking \cit{157, 104, 38, 123}{,} Fairness \cit{173}, leaf2]
            ]
            [\ \ \ Interpretability
                [\eg Linear Rep. Hypothesis \cit{229}{,} Geometry of Truth \cit{206}{,} Reverse Curse \cit{14}{,} Position Bias \cit{320}{,} Induction Heads \cit{220}, leaf2]
            ]
        ]
    ]
\end{forest}
